Structure-Preserving Sparsification Methods for Social Networks

Sparsification reduces the size of networks while preserving structural and statistical properties of interest. Various sparsifying algorithms have been proposed in different contexts. We contribute the first systematic conceptual and experimental comparison of \textit{edge sparsification} methods on a diverse set of network properties. It is shown that they can be understood as methods for rating edges by importance and then filtering globally or locally by these scores. We show that applying a local filtering technique improves the preservation of all kinds of properties. In addition, we propose a new sparsification method (\textit{Local Degree}) which preserves edges leading to local hub nodes. All methods are evaluated on a set of social networks from Facebook, Google+, Twitter and LiveJournal with respect to network properties including diameter, connected components, community structure, multiple node centrality measures and the behavior of epidemic simulations. In order to assess the preservation of the community structure, we also include experiments on synthetically generated networks with ground truth communities. Experiments with our implementations of the sparsification methods (included in the open-source network analysis tool suite NetworKit) show that many network properties can be preserved down to about 20\% of the original set of edges for sparse graphs with a reasonable density. The experimental results allow us to differentiate the behavior of different methods and show which method is suitable with respect to which property. While our Local Degree method is best for preserving connectivity and short distances, other newly introduced local variants are best for preserving the community structure.

==> figures/parameterization_results.tex <==
% --------------- Generated --------------
\begin{tabular}{ll||ll||ll||ll||ll||ll||ll||ll||ll||ll|}
 &  & \multicolumn{2}{c|}{\textbf{$e_t=0.010$}} & \multicolumn{2}{c|}{\textbf{$e_t=0.050$}} & \multicolumn{2}{c|}{\textbf{$e_t=0.100$}} & \multicolumn{2}{c|}{\textbf{$e_t=0.150$}} & \multicolumn{2}{c|}{\textbf{$e_t=0.200$}} & \multicolumn{2}{c|}{\textbf{$e_t=0.300$}} & \multicolumn{2}{c|}{\textbf{$e_t=0.500$}} & \multicolumn{2}{c|}{\textbf{$e_t=0.700$}} & \multicolumn{2}{c|}{\textbf{$e_t=0.900$}} \\ \hline
\textbf{Graph} & \textbf{Backbone} & $p$ & $e$ & $p$ & $e$ & $p$ & $e$ & $p$ & $e$ & $p$ & $e$ & $p$ & $e$ & $p$ & $e$ & $p$ & $e$ & $p$ & $e$ \\ \hline
BTER & ForestFire 1 & 0.453 & 0.007 & 0.195 & 0.041 & 0.117 & 0.080 & 0.086 & 0.119 & 0.062 & 0.172 & 0.039 & 0.280 & 0.023 & 0.441 & 0.016 & 0.595 & 0.008 & 0.811 \\ \hline
BTER & Local Similarity & 0.062 & 0.064 & 0.062 & 0.064 & 0.259 & 0.100 & 0.367 & 0.150 & 0.449 & 0.200 & 0.565 & 0.299 & 0.713 & 0.500 & 0.823 & 0.700 & 0.940 & 0.900 \\ \hline
BTER & Random 1 & 0.010 & 0.010 & 0.050 & 0.050 & 0.100 & 0.100 & 0.150 & 0.150 & 0.200 & 0.202 & 0.300 & 0.300 & 0.500 & 0.498 & 0.700 & 0.698 & 0.900 & 0.898 \\ \hline
BTER & Simmelian Multiscale & 0.368 & 0.010 & 0.368 & 0.050 & 0.369 & 0.100 & 0.369 & 0.151 & 0.369 & 0.200 & 0.369 & 0.300 & 0.370 & 0.500 & 0.373 & 0.702 & 0.382 & 0.896 \\ \hline
BTER & Simmelian NonParametric & 0.996 & 0.404 & 0.996 & 0.404 & 0.996 & 0.404 & 0.996 & 0.404 & 0.996 & 0.404 & 0.996 & 0.404 & 0.971 & 0.499 & 0.945 & 0.696 & 0.889 & 0.901 \\ \hline
BTER & Simmelian Parametric & 10 & 0.552 & 10 & 0.552 & 10 & 0.552 & 10 & 0.552 & 10 & 0.552 & 10 & 0.552 & 10 & 0.552 & 8 & 0.695 & 2 & 0.899 \\ \hline
Caltech36 & ForestFire 1 & 0.156 & 0.009 & 0.062 & 0.051 & 0.051 & 0.081 & 0.039 & 0.143 & 0.035 & 0.199 & 0.031 & 0.280 & 0.016 & 0.723 & 0.012 & 0.723 & 0.008 & 0.877 \\ \hline
Caltech36 & Local Similarity & 0.125 & 0.038 & 0.173 & 0.050 & 0.333 & 0.100 & 0.437 & 0.150 & 0.514 & 0.200 & 0.621 & 0.300 & 0.766 & 0.500 & 0.873 & 0.700 & 0.958 & 0.900 \\ \hline
Caltech36 & Random 1 & 0.010 & 0.011 & 0.050 & 0.050 & 0.100 & 0.100 & 0.150 & 0.151 & 0.200 & 0.197 & 0.300 & 0.296 & 0.500 & 0.501 & 0.700 & 0.693 & 0.900 & 0.903 \\ \hline
Caltech36 & Simmelian Multiscale & 0.369 & 0.015 & 0.369 & 0.050 & 0.369 & 0.098 & 0.369 & 0.142 & 0.369 & 0.198 & 0.369 & 0.298 & 0.370 & 0.504 & 0.370 & 0.701 & 0.372 & 0.899 \\ \hline
Caltech36 & Simmelian NonParametric & 0.969 & 0.149 & 0.969 & 0.149 & 0.969 & 0.149 & 0.922 & 0.150 & 0.689 & 0.200 & 0.530 & 0.300 & 0.332 & 0.504 & 0.176 & 0.700 & 0.091 & 0.899 \\ \hline
Caltech36 & Simmelian Parametric & 10 & 0.005 & 8 & 0.070 & 8 & 0.070 & 7 & 0.143 & 6 & 0.236 & 5 & 0.333 & 3 & 0.544 & 2 & 0.671 & 1 & 0.827 \\ \hline
KitEmail & ForestFire 1 & 0.531 & 0.002 & 0.297 & 0.035 & 0.125 & 0.100 & 0.094 & 0.132 & 0.070 & 0.187 & 0.062 & 0.231 & 0.031 & 0.549 & 0.016 & 0.731 & 0.008 & 0.906 \\ \hline
KitEmail & Local Similarity & 0.062 & 0.106 & 0.062 & 0.106 & 0.062 & 0.106 & 0.287 & 0.150 & 0.396 & 0.200 & 0.541 & 0.300 & 0.716 & 0.500 & 0.837 & 0.700 & 0.942 & 0.900 \\ \hline
KitEmail & Multiscale & 0.000 & 0.013 & 0.003 & 0.050 & 0.035 & 0.100 & 0.107 & 0.150 & 0.195 & 0.200 & 0.373 & 0.300 & 0.633 & 0.500 & 0.810 & 0.700 & 0.928 & 0.900 \\ \hline
KitEmail & Random 1 & 0.010 & 0.012 & 0.050 & 0.052 & 0.100 & 0.106 & 0.150 & 0.151 & 0.200 & 0.200 & 0.300 & 0.301 & 0.500 & 0.499 & 0.700 & 0.696 & 0.900 & 0.899 \\ \hline
KitEmail & Simmelian Multiscale & 0.000 & 0.013 & 0.003 & 0.050 & 0.035 & 0.100 & 0.107 & 0.150 & 0.195 & 0.200 & 0.373 & 0.300 & 0.633 & 0.500 & 0.810 & 0.700 & 0.928 & 0.900 \\ \hline
KitEmail & Simmelian NonParametric & 0.984 & 0.048 & 0.944 & 0.050 & 0.801 & 0.098 & 0.715 & 0.149 & 0.648 & 0.200 & 0.518 & 0.300 & 0.336 & 0.476 & 0.197 & 0.700 & 0.064 & 0.900 \\ \hline
KitEmail & Simmelian Parametric & 10 & 0.037 & 9 & 0.055 & 8 & 0.100 & 7 & 0.175 & 7 & 0.175 & 6 & 0.267 & 4 & 0.463 & 2 & 0.708 & 1 & 0.857 \\ \hline
LFR-1000 & ForestFire 1 & 0.656 & 0.008 & 0.531 & 0.032 & 0.500 & 0.057 & 0.500 & 0.057 & 0.375 & 0.167 & 0.375 & 0.167 & 0.250 & 0.535 & 0.188 & 0.687 & 0.062 & 0.931 \\ \hline
LFR-1000 & Local Similarity & 0.125 & 0.087 & 0.125 & 0.087 & 0.207 & 0.100 & 0.289 & 0.150 & 0.375 & 0.200 & 0.508 & 0.300 & 0.699 & 0.498 & 0.867 & 0.699 & 0.960 & 0.900 \\ \hline
LFR-1000 & Random 1 & 0.010 & 0.011 & 0.050 & 0.049 & 0.100 & 0.103 & 0.150 & 0.153 & 0.200 & 0.204 & 0.300 & 0.302 & 0.500 & 0.497 & 0.700 & 0.694 & 0.900 & 0.900 \\ \hline
LFR-1000 & Simmelian Multiscale & 0.372 & 0.046 & 0.372 & 0.046 & 0.372 & 0.108 & 0.372 & 0.139 & 0.372 & 0.210 & 0.372 & 0.312 & 0.374 & 0.507 & 0.375 & 0.697 & 0.379 & 0.903 \\ \hline
LFR-1000 & Simmelian NonParametric & 0.938 & 0.156 & 0.938 & 0.156 & 0.938 & 0.156 & 0.938 & 0.156 & 0.703 & 0.199 & 0.516 & 0.283 & 0.301 & 0.499 & 0.060 & 0.700 & 0.022 & 0.898 \\ \hline
LFR-1000 & Simmelian Parametric & 10 & 0.006 & 8 & 0.061 & 7 & 0.110 & 7 & 0.110 & 6 & 0.191 & 5 & 0.297 & 3 & 0.530 & 1 & 0.710 & 0 & 1.000 \\ \hline
PGP & ForestFire 1 & 0.625 & 0.012 & 0.469 & 0.065 & 0.406 & 0.112 & 0.344 & 0.176 & 0.312 & 0.176 & 0.188 & 0.362 & 0.125 & 0.501 & 0.062 & 0.719 & 0.031 & 0.868 \\ \hline
PGP & Local Similarity & 0.125 & 0.369 & 0.125 & 0.369 & 0.125 & 0.369 & 0.125 & 0.369 & 0.125 & 0.369 & 0.125 & 0.369 & 0.459 & 0.501 & 0.682 & 0.697 & 0.877 & 0.900 \\ \hline
PGP & Random 1 & 0.010 & 0.010 & 0.050 & 0.049 & 0.100 & 0.103 & 0.150 & 0.148 & 0.200 & 0.198 & 0.300 & 0.297 & 0.500 & 0.498 & 0.700 & 0.695 & 0.900 & 0.899 \\ \hline
PGP & Simmelian Multiscale & 0.369 & 0.008 & 0.370 & 0.051 & 0.371 & 0.100 & 0.372 & 0.148 & 0.372 & 0.201 & 0.374 & 0.296 & 0.379 & 0.492 & 0.391 & 0.688 & 0.438 & 0.911 \\ \hline
PGP & Simmelian NonParametric & 0.984 & 0.198 & 0.984 & 0.198 & 0.984 & 0.198 & 0.984 & 0.198 & 0.970 & 0.200 & 0.781 & 0.298 & 0.500 & 0.507 & 0.199 & 0.715 & 0.063 & 0.898 \\ \hline
PGP & Simmelian Parametric & 10 & 0.093 & 10 & 0.093 & 10 & 0.093 & 9 & 0.133 & 7 & 0.218 & 5 & 0.316 & 3 & 0.461 & 2 & 0.603 & 1 & 0.877 \\ \hline
Tennessee95 & ForestFire 1 & 0.070 & 0.008 & 0.035 & 0.038 & 0.025 & 0.081 & 0.020 & 0.129 & 0.020 & 0.129 & 0.016 & 0.220 & 0.010 & 0.393 & 0.008 & 0.523 & 0.002 & 0.951 \\ \hline
Tennessee95 & Local Similarity & 0.062 & 0.018 & 0.289 & 0.050 & 0.434 & 0.100 & 0.522 & 0.150 & 0.586 & 0.200 & 0.680 & 0.300 & 0.806 & 0.500 & 0.894 & 0.700 & 0.963 & 0.900 \\ \hline
Tennessee95 & Random 1 & 0.010 & 0.010 & 0.050 & 0.050 & 0.100 & 0.100 & 0.150 & 0.150 & 0.200 & 0.200 & 0.300 & 0.300 & 0.500 & 0.500 & 0.700 & 0.700 & 0.900 & 0.900 \\ \hline
Tennessee95 & Simmelian Multiscale & 0.368 & 0.010 & 0.368 & 0.050 & 0.368 & 0.100 & 0.368 & 0.151 & 0.368 & 0.201 & 0.369 & 0.299 & 0.369 & 0.500 & 0.369 & 0.702 & 0.370 & 0.899 \\ \hline
Tennessee95 & Simmelian NonParametric & 0.992 & 0.089 & 0.992 & 0.089 & 0.854 & 0.100 & 0.664 & 0.153 & 0.528 & 0.200 & 0.334 & 0.291 & 0.146 & 0.500 & 0.067 & 0.700 & 0.024 & 0.900 \\ \hline
Tennessee95 & Simmelian Parametric & 9 & 0.008 & 7 & 0.052 & 6 & 0.095 & 5 & 0.147 & 4 & 0.208 & 3 & 0.277 & 1 & 0.575 & 1 & 0.575 & 0 & 1.000 \\ \hline
USAviation & ForestFire 1 & 0.398 & 0.012 & 0.203 & 0.048 & 0.141 & 0.087 & 0.094 & 0.147 & 0.078 & 0.174 & 0.047 & 0.315 & 0.031 & 0.541 & 0.016 & 0.717 & 0.008 & 0.894 \\ \hline
USAviation & Local Similarity & 0.062 & 0.072 & 0.062 & 0.072 & 0.248 & 0.100 & 0.376 & 0.150 & 0.462 & 0.200 & 0.583 & 0.300 & 0.732 & 0.500 & 0.834 & 0.700 & 0.927 & 0.900 \\ \hline
USAviation & Multiscale & 0.000 & 0.010 & 0.002 & 0.050 & 0.013 & 0.100 & 0.045 & 0.150 & 0.100 & 0.200 & 0.294 & 0.300 & 0.656 & 0.500 & 0.822 & 0.700 & 0.917 & 0.900 \\ \hline
USAviation & Random 1 & 0.010 & 0.010 & 0.050 & 0.047 & 0.100 & 0.103 & 0.150 & 0.146 & 0.200 & 0.200 & 0.300 & 0.305 & 0.500 & 0.497 & 0.700 & 0.702 & 0.900 & 0.900 \\ \hline
USAviation & Simmelian Multiscale & 0.000 & 0.010 & 0.002 & 0.050 & 0.013 & 0.100 & 0.045 & 0.150 & 0.100 & 0.200 & 0.294 & 0.300 & 0.656 & 0.500 & 0.822 & 0.700 & 0.917 & 0.900 \\ \hline
USAviation & Simmelian NonParametric & 0.984 & 0.149 & 0.984 & 0.149 & 0.984 & 0.149 & 0.974 & 0.150 & 0.866 & 0.200 & 0.752 & 0.292 & 0.579 & 0.500 & 0.416 & 0.702 & 0.193 & 0.900 \\ \hline
USAviation & Simmelian Parametric & 10 & 0.022 & 9 & 0.065 & 9 & 0.065 & 8 & 0.163 & 8 & 0.163 & 7 & 0.297 & 6 & 0.442 & 4 & 0.690 & 2 & 0.880 \\ \hline
Virginia63 & ForestFire 1 & 0.086 & 0.011 & 0.047 & 0.052 & 0.033 & 0.101 & 0.035 & 0.101 & 0.023 & 0.225 & 0.020 & 0.301 & 0.012 & 0.533 & 0.008 & 0.685 & 0.002 & 0.952 \\ \hline
Virginia63 & Local Similarity & 0.062 & 0.025 & 0.243 & 0.050 & 0.395 & 0.100 & 0.488 & 0.150 & 0.557 & 0.200 & 0.656 & 0.300 & 0.791 & 0.500 & 0.887 & 0.700 & 0.961 & 0.900 \\ \hline
Virginia63 & Random 1 & 0.010 & 0.010 & 0.050 & 0.050 & 0.100 & 0.100 & 0.150 & 0.150 & 0.200 & 0.200 & 0.300 & 0.299 & 0.500 & 0.499 & 0.700 & 0.701 & 0.900 & 0.900 \\ \hline
Virginia63 & Simmelian Multiscale & 0.368 & 0.010 & 0.368 & 0.050 & 0.368 & 0.100 & 0.369 & 0.150 & 0.369 & 0.200 & 0.369 & 0.300 & 0.369 & 0.500 & 0.370 & 0.698 & 0.371 & 0.900 \\ \hline
Virginia63 & Simmelian NonParametric & 0.992 & 0.119 & 0.992 & 0.119 & 0.992 & 0.119 & 0.789 & 0.150 & 0.631 & 0.200 & 0.384 & 0.300 & 0.154 & 0.499 & 0.062 & 0.701 & 0.022 & 0.900 \\ \hline
Virginia63 & Simmelian Parametric & 10 & 0.005 & 8 & 0.042 & 7 & 0.078 & 5 & 0.175 & 5 & 0.175 & 3 & 0.297 & 1 & 0.588 & 1 & 0.588 & 0 & 1.000 \\ \hline
Yale4 & ForestFire 1 & 0.066 & 0.010 & 0.031 & 0.047 & 0.020 & 0.109 & 0.018 & 0.144 & 0.016 & 0.195 & 0.014 & 0.271 & 0.008 & 0.522 & 0.006 & 0.691 & 0.004 & 0.851 \\ \hline
Yale4 & Local Similarity & 0.062 & 0.017 & 0.300 & 0.050 & 0.446 & 0.100 & 0.535 & 0.150 & 0.600 & 0.200 & 0.694 & 0.300 & 0.818 & 0.500 & 0.901 & 0.700 & 0.967 & 0.900 \\ \hline
Yale4 & Random 1 & 0.010 & 0.010 & 0.050 & 0.050 & 0.100 & 0.100 & 0.150 & 0.150 & 0.200 & 0.200 & 0.300 & 0.299 & 0.500 & 0.501 & 0.700 & 0.699 & 0.900 & 0.900 \\ \hline
Yale4 & Simmelian Multiscale & 0.368 & 0.010 & 0.368 & 0.050 & 0.368 & 0.100 & 0.368 & 0.150 & 0.368 & 0.202 & 0.369 & 0.302 & 0.369 & 0.498 & 0.369 & 0.698 & 0.370 & 0.901 \\ \hline
Yale4 & Simmelian NonParametric & 0.984 & 0.141 & 0.984 & 0.141 & 0.984 & 0.141 & 0.750 & 0.151 & 0.504 & 0.197 & 0.334 & 0.281 & 0.167 & 0.501 & 0.084 & 0.700 & 0.036 & 0.900 \\ \hline
Yale4 & Simmelian Parametric & 8 & 0.015 & 7 & 0.036 & 5 & 0.117 & 4 & 0.178 & 4 & 0.178 & 3 & 0.258 & 1 & 0.621 & 1 & 0.621 & 0 & 1.000 \\ \hline
\end{tabular}
% --------------- Generated --------------

